Inductive or Deductive? Rethinking the Fundamental Reasoning Abilities of LLMs

Reasoning encompasses two typical types: deductive reasoning and inductive reasoning. Despite extensive research into the reasoning capabilities of Large Language Models (LLMs), most studies have failed to rigorously differentiate between inductive and deductive reasoning, leading to a blending of the two. This raises an essential question: In LLM reasoning, which poses a greater challenge - deductive or inductive reasoning? While the deductive reasoning capabilities of LLMs, (i.e. their capacity to follow instructions in reasoning tasks), have received considerable attention, their abilities in true inductive reasoning remain largely unexplored. To investigate into the true inductive reasoning capabilities of LLMs, we propose a novel framework, SolverLearner. This framework enables LLMs to learn the underlying function (i.e., $y = f_w(x)$), that maps input data points $(x)$ to their corresponding output values $(y)$, using only in-context examples. By focusing on inductive reasoning and separating it from LLM-based deductive reasoning, we can isolate and investigate inductive reasoning of LLMs in its pure form via SolverLearner. Our observations reveal that LLMs demonstrate remarkable inductive reasoning capabilities through SolverLearner, achieving near-perfect performance with ACC of 1 in most cases. Surprisingly, despite their strong inductive reasoning abilities, LLMs tend to relatively lack deductive reasoning capabilities, particularly in tasks involving ``counterfactual'' reasoning.

==> content/discussion.tex <==
\section{Discussion}\label{sec:discussion}

\textbf{Why might we prefer to teach a model instead of directing the reasoning of a Large Language Model (LLM) through in-context learning?}
Guiding the reasoning of a LLM through in-context learning can indeed face challenges, such as the risk of hallucinations. Even state-of-the-art LLMs exhibit limitations in various domains. For instance, these models are susceptible to inaccuracies in arithmetic calculations, especially when handling large numerical values, primarily because they do not rely on strict computational precision, as observed in previous studies~~\cite{}. Another open challenge for LLMs is that they often experience a notable decline in accuracy when dealing with tasks that deviates from conventional knowledge~\cite{wu2023reasoning}. These observations have led several academic papers to conclude that the achievements of existing LLMs should not be entirely attributed to their general capacity for the target task, but rather they tend to perform by rote memorization. Our current study demonstrates that LLMs possess the ability to discern common patterns among various instances, even when tackling tasks that depart from conventional knowledge. However, harnessing this capability and distilling the knowledge it accumulates requires a deliberate approach. For instance, we advocate for the distillation of a model to compel LLMs to genuinely comprehend content and systematically encode patterns, instead of merely emulating behavior based on a few-shot examples. Additionally, for computationally intensive tasks, the delegation of computational steps to an external ``calculator'' serves as a viable strategy to address the issue of hallucinations.

\textbf{What advantages do we gain from using LLMs for solver learner in comparison to machine learning methods?}
Pattern learning helps in discovering underlying structures and relationships in data, providing insights that might not be immediately apparent. By identifying patterns, we can make predictions about future events, trends, or behaviors. This is crucial in fields like finance, healthcare, marketing, and many others. The existing works span from traditional rule learning techniques to advanced machine learning approaches.
Traditional rule learning methods, while valuable, have limitations in expressiveness, as they require explicit rule definitions and prior domain knowledge typically represented in logical forms. Preparing such data is labor-intensive, and the domain knowledge is often constrained, failing to cover all aspects of the world. In contrast, LLMs inherently encode world knowledge within their parameters, setting them apart from traditional rule learning approaches.


% Machine learning, while powerful in the field of pattern learning, are often considered ``black boxes'' due to their complex structure. Understanding why and how these models make certain decisions can be challenging, which is a significant drawback in fields where explainability is critical, such as healthcare and finance. 

\section{Open Problems}\label{sec:open problem}
Given the vast potential of this field, it is clear that much remains to be explored and understood:

\textbf{The scope: Identifying the Types of Problems Solvable by LLMs}
The majority of tasks examined in our experiments involve a relatively straightforward mapping function $f$ to establish a relationship between $(x,y)$. However, certain problems may be excessively intricate or fundamentally unpredictable, posing challenges to effective generalization. For instance, is it feasible for LLMs to address issues characterized by complex many-to-many mapping functions? Determining the specific range of problems that can be effectively tackled by LLMs is a critical inquiry. Additionally, quantifying the complexity of a problem and understanding the threshold of complexity that LLMs can successfully handle remains an area of exploration.

\textbf{Assessing Training Data Adequacy: Measuring the Quality of Learning Inputs}
% \KC{difficulty of the function}
The accuracy of the hypothesis learning is heavily dependent on the quality of the observed data. In situations where training relies on a limited number of examples, commonly known as 'few-shot' learning, the representativeness of these examples becomes significant. Insufficient or non-representative data can hinder the ability of Large Language Models (LLMs) to generalize and make precise predictions on new data. The complexity of the task being tackled determines the minimum number of few-shot examples required for effective training. Quantifying this minimum requirement constitutes a critical research area. Similarly, the diversity within the training dataset is equally significant.

\textbf{Validating Learning Hypotheses: A Challenge in Science and Our Setting}
Evaluating the correctness of a learning hypothesis is a complex issue, prevalent in both scientific and machine learning domains. Even well-established hypotheses and theories are subject to revision or rejection in the light of new evidence. The primary objective in science is not to prove a hypothesis absolutely correct, but rather to rigorously test and understand its validity. This principle holds true in our context of LLMs. An essential yet challenging aspect is fostering an authentic self-discussion about the problem within LLMs, ensuring that these models not only retrieve the underlying pattern but also reflect an inspiring understanding of the learned hypothesis.

We hope that this research serves as an inspiration and foundation for further studies in these areas, paving the way for more refined and effective uses of LLMs in the future.

% \textbf{What will be the best way to encode learned pattern?}
% Encoding rules in computational models is a crucial aspect of various AI systems. First-order logic (FOL) has been widely used as the formal language for rule representation in the domain of AI. However, it also has certain limitations. First of all, FOL can be quite complex, both in terms of its syntax and semantics. Writing and understanding FOL statements, especially complex ones, requires a good grasp of formal logic principles, which can be a barrier for those not well-versed in these areas. Second, it is can only make decisions based on the rules provided. they can also generate trivial or irrelevant rules.

% Neural Network can also 
% % Logical systems often assume complete and accurate information, but in the real world, information is often incomplete, uncertain, or ambiguous. This makes it challenging to apply precise logical rules directly to situations where all the relevant information is not available.

% Although nature language itself could be powerful enough to describe any situation but it usually suffer from severe ambiguity. We have discussed the performance of directly encoding the rule in nature language in Sec~\ref{sec:Results} Therefore, we suggest to employ code to encode rule as it is precise and 

==> content/insight.tex <==
% \section{Insights and Understanding}
\section{Comparing Our Insights with Existing Research}
% The goal of the \model{} project is to really dig into what LLMs can do – basically, to find out how far their abilities can go. We did a bunch of tests and what we found is pretty interesting: these models are actually pretty good at thinking in a more abstract way. This means they're not just stuck by reciting the seen examplar, but can actually see patterns that are common across different examplars. It's like they're learning to apply what they know to new situations, which is a big step forward in making them more useful for different kinds of problems. The \model{} project helps us understand more about how these language models are getting better and more versatile.
The concept of ``inductive reasoning'' discussed in this paper differs from its typical usage in the context of Inductive Logic Programming (ILP). In ILP, inductive reasoning is employed to derive logical rules from observational data, given the background knowledge.
These rules are typically formulated in First-Order Logic. In contrast, our approach involves leveraging pre-existing knowledge embedded within LLMs in a creative manner. The objective here is to establish a consistent mapping function that logically connects input to output, based on observational data. Our study focuses on evaluating the ability of a LLMs to engage in divergent thinking. This process involves starting from a variety of instances and methodically working towards identifying a unifying pattern that links these disparate elements. The emphasis is on understanding how a LLM can navigate and connect diverse pieces of information to arrive at coherent conclusions.


==> content/method_old.tex <==
\section{Our Framework: \model{}}
\begin{figure*}[h]
    % \vspace{-0.2in}
    \centering
    \includegraphics[width= \linewidth]{figure/framework.pdf}
    %\vspace{-2em}
    \caption{An overview of the proposed framework, \textit{\model{}}. } 
    \label{fig:framework}
% \vspace{-0.2in}
\end{figure*}

The scientific research method typically follows these steps: (1) Observation and Problem Definition: Begins with observing natural or experimental phenomena, proposing and defining a formal research problem; (2) Literature Review and Hypothesis Proposal: Involves reviewing relevant studies to propose a testable hypothesis; (3) Experimental Design: Developing experiments to test the hypothesis; (4) Verification and Improvement: Conducting experiments to confirm or refute the hypothesis and refining it based on the results. Inspired by the method of scientific research, we proposed a framework enabling LLMs to learn and and evaluate hypotheses, as illustrated in Fig~\ref{fig:framework}. The process involves:
\begin{itemize}
    \item \textbf{Few-Shot Examples Preparation and Problem Definition:} Users provide background information and few-shot examples as $(x, y)$ pairs, detailed in the Appendix~\ref{app:Prompts}. 
    \item \textbf{Literature Review and Hypothesis Proposal:} LLMs naturally access relevant literature (e.g., activating the associated neuron) and derive a shared hypothesis based on the given examples accordingly.
    \item \textbf{Experimental Design:} Transform the learned patterns into a testable format, such as a Python program. 
    \item \textbf{Verification and Self-improvement:} Use the created design or program to test the hypothesis against the few-shot examples, refining as needed.
\end{itemize}

\subsection{Framework}
In this subsection, we will take the two-digit addition task as a case study to demonstrate the entire process.
% The scientific research method usually involves several key steps: (1) observation and problem definition: scientific research often begins with observations of the natural world or experimental phenomena, leading to the formal formulation of research problems. (2) literature review and hypothesis: : researchers review existing knowledge in the field by reading relevant studies and materials. (3) hypothesis: based on observations and literature review, a testable hypothesis is proposed. (4) experimental design: experiments are designed to test the hypothesis. This may include design a systematic way to test each sample. (5) Verification and self improve. Verify the observation via experiments to determine whether they support or refute the hypothesis. Based on the results, improve the hypothesis.
% Following such principle, we proposed a framework designed to allow LLMs to learn and verify hypothesis in a systematic way. This framework consists of two key phases: (1) few-shot examples preparation and problem definition: this is the input of the framework, the user require to provide necessary background to define the problem and  prepare few-shot in form of pairs of $(x, y)$. We have provide examples of the input of the framework in the appendix. (2) literature review and hypothesis proposal, given the input, LLMs naturally have the ability to retrieve all related literature (e.g., activate corresponding neuron) and proposed the most common shared hypothesis related to all few shot examples. (3) experimental design: convert the learn pattern into a way (e.g., Python program) to be able system test the hypothesis over the few shot example.  (4) Verification and self improve. The generated experimental design (e.g., Python program) is used to verify over the few shot example to determine support or refute the hypothesis.

\textbf{Few-Shot Examples Preparation and Problem Definition:}
To facilitate LLMs in learning patterns from few-shot examples, it is crucial to provide a precise Problem Definition to confine the issue within a manageable scope. Without restricting the problem to a more focused area, formulating an accurate Hypothesis becomes challenging. This is because, in the absence of any constraints, there could be numerous explanations for the few-shot examples. For instance, the two-digit addition task in our experiment can be defined as follows, accompanied by a few examples:

\textit{``You are an expert mathematician and programmer. You are asked to add two numbers, the base of which is unknow. Below are some provided examples:\\
The result for 76+76 is 174. ... The result for 75+41 is 136.\\
Please identify the underlying pattern to determine the base being used.''}

\textbf{Literature Review and Hypothesis Proposal:} 
Considering the provided background information and few-shot examples, the objective for LLMs is to generate a hypothesis that explain all examples, akin to the hypothesis formulation stage in scientific research. An intuitive explanation for why LLMs can generalize from few-shot examples is their proficiency in detecting correlations between tokens or clusters of tokens. As explored in~\cite{billslanguage}, common patterns in few-shot examples may activate the same group of neurons in LLMs. This collective neuron activation might contribute to the recognition of a unified hypothesis. This approach is distinct from conventional scientific research that explore unknown domains. Instead, LLMs achieve generalization by retrieving and establishing connections among instances and existing hypotheses.

\textbf{Experimental Design:}
After learning the hypothesis, it's important to conduct experiments to validate it. Although this process may seem straightforward, it involves more than just letting the LLMs directly solve problems based on learned rules, as previous works have done~\cite{wu2023reasoning}. A key characteristic of scientific experiments is accuracy and reproducibility. Given the inherent randomness of LLMs and the ambiguity of language, they are not ideal for conducting experiments. Fortunately, tools such as computers can serve as perfect executors for these experiments. For example, while it may not be trivial to translate the task of solving a two-digit addition problem into an implementable process, we can encode this task into Python code for experimental design purposes. In designing experiments for the two-digit addition task, we have:

\textit{``Please identify the underlying pattern to determine the base being used and implement a solver() function to achieve the goal. \\
def solver(n1: str, n2: str) -> str:\\
    \# Let's write a Python program step by step\\
    \# Each input is a number represented as a string.\\
    \# The function computes the sum of these numbers and returns it as a string.\\
After defining the solver() function, create test cases based on the input examples and print the results. An example of a test case could be ``print(solver(``76'', ``76''))''.''}

\textbf{Verification and Self-improvement:}
Verification and self-improvement are critical steps in scientific research. This phase tests the hypothesis against few-shot examples through experiments. By analyzing the correctly identified examples and learning from the mistakes in incorrectly identified ones, scientists refine their hypotheses for improvement. Similarly, our framework includes a verification and self-improvement stage. In this phase, the experimental results are fed back to the LLMs, allowing them to refine their hypothesis. This iterative process is repeated until the accuracy on the validation dataset reaches a predetermined threshold. For example, the verification of the two-digit addition task for base 9 is described as follows:

\textit{``The generated code is:\\
def solver(n1: str, n2: str) -> str:\\
    \# From the given examples, we can infer that the base being used is 9 \\
    base = 9 \\
    \# Convert the input strings to integers in base 9 \\
    num1 = int(n1, base) \\
    num2 = int(n2, base) \\
    \# Calculate the sum of the numbers \\
    result = num1 + num2 \\
    \# Convert the result back to a string in base 9 \\
    return format(result, f'X').replace("A", "10").replace("B", "11").replace("C", "12").replace("D", "13").replace("E", "14").replace("F", "15") \\ 
\# Test cases \\
print(solver("76", "14"))  \# Expected output: 101 \\
...\\
print(solver("85", "45"))  \# Expected output: 141 \\
By running the generated program against the test cases, the following 0 test cases are correctly predicted: \\
$[]$\\
Meanwhile, 8 test cases result in incorrect predictions. Below, we present both the correct answers and the erroneous predictions for these incorrect test cases:\\
The answer for print (solver("76","14")) is expected to be 101. However, the prediction is incorrect, as evidenced by the following result: 52\\
...\\
The answer for print (solver("85","45")) is expected to be 141. However, the prediction is incorrect, as evidenced by the following result: 76 \\
Please rectify the learned pattern and improve the solver() function to address the inaccurate test cases.''}

